Data Generation for Testing Complex Queries

Generation of sample data for testing SQL queries has been an important task for many years, with applications such as testing of SQL queries used for data analytics and in application software, as well as student SQL queries. More recently, with the increasing use of text-to-SQL systems, test data is key for the validation of generated queries. Earlier work for test data generation handled basic single block SQL queries, as well as simple nested SQL queries, but could not handle more complex queries. In this paper, we present a novel data generation approach that is designed to handle complex queries, and show its effectiveness on queries for which the earlier XData approach is not as effective. We also show that it can outperform the state-of-the-art VeriEQL system in showing non-equivalence of queries.

==> sections/nullsComp.tex <==



%Enumerated datatypes of the constraint solver are used to represent string attributes.
%XData \cite{xdata2015} uses CVC3 constraints solver which support non-equal comparision of enumerated datatypes.
%As per our knowledge, Z3 does not support comparison operators for enumerated datatypes except for equal to. To model selection conditions such as \verb|Attr1 relop Attr2|; where Attr1 and Attr2 are string type variables, we use user-defined comparison operation i.e. greater than and less than For pair of values \verb|a1, a2| in domain, we assert a function gt\_attr.  We sort the values in the attributes's domain lexicographically descending order. Then for each pair \verb|v1 > v2| we call \verb|gt_attr| function.

%\begin{algorithm}[H]
%\caption{Define greater than function for attribute }
%\label{isValid}
%\begin{algorithmic}[1]
%    \Function {gtAttr } {attr a1, attr a2}
%    \State \hspace{5mm} a1 $\neq$ a2
%    \State \hspace{5mm} not \Call{gtAttr}{a2, a1} 
%    \EndFunction
%\State \textbf{assert}
%\State \hspace{5mm} \Call{gtAttr}{v1, v2}
%\State \hspace{5mm} \Call{gtAttr}{v2, v3} 
%$\ldots$
%\end{algorithmic}
%\end{algorithm}

% A similar function is defined for less than by sorting the attribute values in lexicographically ascending order. This allows us to support \verb|Attr1 relop Attr2| in return, killing non-equi join mutations. 

%To handle string condition of format \verb|Attr1 relop |\verb|"value"|, XData \cite{xdata2015} uses their own string solver to solve the constraints, especially when the relop is non-equal comparision operator. String solver first finds a suitable string value i.e. \verb|solved_value| for the attributed based on the condition, then converts \verb|Attr1 relop "value"| into \verb|Attr1 = "solved_value"|. This method restricts the possible value that the attribute can have. We utilize XData's string solver to identify one or more string values, incorporate these into the attribute's range, while maintaining the original string constraints intact. This approach grants the solver flexibility in selecting values.

==> sections/numberoftuples.tex <==


